CTDS: Centralized Teacher with Decentralized Student for Multi-Agent Reinforcement Learning

Due to the partial observability and communication constraints in many multi-agent reinforcement learning (MARL) tasks, centralized training with decentralized execution (CTDE) has become one of the most widely used MARL paradigms. In CTDE, centralized information is dedicated to learning the allocation of the team reward with a mixing network, while the learning of individual Q-values is usually based on local observations. The insufficient utility of global observation will degrade performance in challenging environments. To this end, this work proposes a novel Centralized Teacher with Decentralized Student (CTDS) framework, which consists of a teacher model and a student model. Specifically, the teacher model allocates the team reward by learning individual Q-values conditioned on global observation, while the student model utilizes the partial observations to approximate the Q-values estimated by the teacher model. In this way, CTDS balances the full utilization of global observation during training and the feasibility of decentralized execution for online inference. Our CTDS framework is generic which is ready to be applied upon existing CTDE methods to boost their performance. We conduct experiments on a challenging set of StarCraft II micromanagement tasks to test the effectiveness of our method and the results show that CTDS outperforms the existing value-based MARL methods.

==> main_body_new.tex <==
\section{Method}
In this section, we first explain the motivation of our proposed framework and introduce the main components in detail.
Besides, we give a theoretical analysis about why our method works.
\subsection{The CTDS Framework}
In this subsection, we present a new framework called Centralized Teacher with Decentralized Student (CTDS), which leverages the idea of knowledge distillation to balance the advantage of global observation and the requirement of decentralized execution.


Recall that in a cooperative multi-agent system, a group of agents coordinate with each other to take joint actions based on the global state information and will obtain a team reward correspondingly.
To achieve decentralize execution, existing CTDE framework requires the individual Q-values in the lower layer only conditioned on the local action-observation histories, and incorporates the state information into mixing network to integrate the individual Q-values into the overall Q-value function.
Obviously, if an agent could have full observation of other agents, it would be more likely to learn a better policy under the cooperative scenario.
Considering the benefit of centralized observations during training, our CTDS decouples the centralized training and decentralized execution with the combination of the teacher module and the student module, as illustrated in Figure~\ref{CTDS}.
% Unlike the previous CTDE framework, CTDS has a teacher module and a student module.
The teacher module is dedicated to allocating the team reward through centralized training, while the student module utilizes the partial observations to approximate the individual Q-value estimated by the teacher model.
In the following, we will give a detailed description about the design of the teacher module and student module, and the knowledge distillation mechanism between them, respectively.

\begin{algorithm}[!] 
	\caption{CTDS Framework.}  
	\label{algo:framework}  
	\begin{algorithmic}[1]
	\REQUIRE the discount factor $\gamma$, the number of agents $N$, the maximum steps $t_{max}$ and target network update period $I$;
	\ENSURE the individual student network;
        \STATE Initialize replay memory $D$, set $t_{step}=0$;
        \STATE Initialize the teacher network, target teacher network and student network with random parameters;
% 		\STATE Initialize the teacher network with random parameters $[\theta_{i},\theta_{mix}]^N_{i=1}$, initialize the student network with random parameters $[\theta_{stu,i}]^N_{i=1}$;
% 		\STATE Initialize the target teacher network with parameters $[\theta_{i}^{-}]^N_{i=1}=[\theta_{i}]^N_{i=1}$, $\theta_{mix}^{-}=\theta_{mix}$;
		\WHILE{$t_{step} \le t_{max}$} % each episode
		    \STATE For each episode, observe initial centralized observation $[\hat{o}^0_i]^N_{i=1}$ and initial decentralized observation $[o^0_i]^N_{i=1}$;
		    \STATE set $t=0$;
		    \WHILE{Not terminal}
		        \STATE With probability $\epsilon$ select a random action $a_i^t$, otherwise $a_i=\mathop{\arg\max}_{a_i^t} Q_i(\hat{\tau}_i^t,a_i^t)$ for each agent $i$;
		        \STATE Take action $\bm{a}^t$ and retrive reward $r_t$, centralized observation $[\hat{o}^{t+1}_i]^N_{i=1}$ and decentralized observation $[o^{t+1}_i]^N_{i=1}$;
		        \STATE $t \leftarrow t+1$;
		    \ENDWHILE
            \STATE $t_{step} \leftarrow t_{step}+t$;
            \STATE Insert the current episode data into buffer $D$;  
		    \STATE Sample a random episode minibatch of transitions $(\bm{\hat{\tau}}, \bm{\tau}, \bm{a}, r, \bm{\hat{\tau}}')$ from $D$;
		    \STATE Set joint action-value $$Q_{tot}=f([Q_i(\hat{\tau}_i,a_i)]^N_{i=1});$$
		    \STATE Set target joint action-value $$Q_{tot}^-=f^-([Q_i^-(\hat{\tau}'_i,\hat{a}_i)]^N_{i=1}),$$where $\hat{a}_i=\arg\max_{a_i}Q_i(\hat{\tau}_i,a_i|\theta_{i})$;
		    \STATE Update the teacher network parameters with TD error $$L_{TD}=(r+\gamma Q_{tot}^- - Q_{tot})^2;$$
		    \STATE Update the student network parameters with distillation loss $$L_{dis}=(Q_i(\hat{\tau}_i,a_i)-Q_{stu,i}(\tau_i,a_i))^2;$$
		    \STATE Update target teacher network parameters with period $I$;
		  %  \STATE Set $Q_{tot}=f([Q_i(\hat{\tau}_i,a_i|\theta_i)]^N_{i=1}|\theta_{mix})$;
		  %  \STATE Set $Q_{tot}^-=f^-([Q_i^-(\hat{\tau}'_i,\hat{a}_i|\theta^-_i)]^N_{i=1}|\theta^-_{mix})$, where $\hat{a}_i=\arg\max_{a_i}Q_i(\hat{\tau}_i,a_i|\theta_{i})$;
		  %  \STATE Update the teacher network parameters $[\theta_{i},\theta_{mix}]^N_{i=1}$ with $L_{td}=(r+\gamma Q_{tot}^- - Q_{tot})^2$;
		  %  \STATE Update the student network parameters $[\theta_{stu,i}]^N_{i=1}$ with $L_{dis}=(Q_i(\hat{\tau}_i,a_i|\theta_i)-Q_{stu,i}(\tau_i,\hat{a}_i|\theta_{stu,i}))^2$;
		  %  \STATE Update target teacher network parameters $[\theta_{i}^{-}]^N_{i=1}=[\theta_{i}]^N_{i=1}$ and $\theta_{mix}^{-}=\theta_{mix}$ with period I;
		\ENDWHILE
	\end{algorithmic}  
\end{algorithm} 

\subsubsection{Teacher Module}
The teacher module consists of two parts: one is the Q-network for estimating individual action-value function for each agent; another is the mixing network for integrating the individual Q-values to be the centralized Q-value.
Note that the teacher module only participates in the centralized training.

The teacher module allows that each agent has an infinite sight range to receive the observation of all the agents.
% In other words, each agent receives the centralized observation $\hat{o}_i$, which complements the missing information in partial observation $o_i$.
% 这里也可以举个例子来说一下$\hat{o}_i$ 和 $o_i$的区别
% Specifically, the teacher module assumes that each agent has an infinite sight range, and completes the missing information in partial observation $o_i$ of each agent.
% For each agent $i$, an individual action-value function $\hat{Q}_i$ is represented by a Q-network, which takes the centralized observation $\hat{o}_i^t$, last action $a_i^{t-1}$ and last hidden state $\hat{h^{t-1}_i}$ as inputs, fits the perfect individual action-value $\hat{Q}_i(\hat{\tau_i},\cdot)$ through the multi-layer perceptron (MLP) and gated recurrent unit (GRU) modules, and outputs the optimal action-value $\hat{Q}_i(\hat{\tau_i},a_i^t)$.
For each agent $g_i$, the Q-network takes the centralized observation $\hat{o}_i^t$, last action $a_i^{t-1}$ and last hidden state $\hat{h}^{t-1}_i$ as inputs, fits the perfect individual action-value $\hat{Q}_i(\hat{\tau}_i,\cdot)$ through the multi-layer perceptron (MLP) and gated recurrent unit (GRU) modules, and outputs the optimal action-value $\hat{Q}_i(\hat{\tau}_i,a_i^t)$.
% Then the centralized observation $\hat{o}_i$ and last action $a_i$ through the MLP and GRU modules to fit perfect individual action-value $\hat{Q}_i$.
% Given the perfect individual action-value $\hat{Q}_i(\hat{\tau_i},a_i^t)$, the teacher module utilizes the mixing network $f$ to combine these individual Q-values into the joint action-value function $\hat{Q}_{tot}$.
Given the perfect individual action-value $\hat{Q}_i(\hat{\tau}_i,a_i^t)$, the mixing network $f$ combines these individual Q-values into the joint action-value function $\hat{Q}_{tot}$ by utilizing the global state information.
% The teacher module combine the perfect individual action-value $\hat{Q}_i$ with the mixing network $f$ to fit the perfect joint action-value $\hat{Q}_{tot}$.
The parameters of the teacher module are updated by the TD loss defined in equation~\ref{eq:TD} iteratively.
% Finally, the same TD loss as the previous CTDE algorithm is calculated to update the parameters of the teacher module.

\subsubsection{Student Module}
To achieve decentralized execution, the agent $g_i$ in the student module only has access to partial observation $o_i^t$, different from the full observation $\hat{o}_i^t$ in the teacher module.
% The student module aims to mimic the output of the teacher module with limited information as much as possible.
Compared with the teacher module, the student module only contains the Q-network, which has the same network architecture as the one in the teacher module but the parameters of Q-networks are not shared.
% Note that the student module adopts the same Q-network in terms of network architecture but the parameters of Q-networks are not shared.
Similarly, the Q-network takes the partial observation $o_i^t$, last action $a_i^{t-1}$ and last hidden state $h^{t-1}_i$ as inputs, and generates the individual action-value $Q_i(\tau_i,\cdot)$ through the MLP and GRU modules.
It can be seen that the student module does not involve any global information and has a relatively simple network structure.
% In the student module, partial observation $o_i$ and last action $a_i$ fit individual action-value $Q_i$ by the MLP and GRU modules with the same structure as the teacher module.
% teacher网络输出来的hot{Q_i}作为label，用MSE loss让Q_i逼近hot{q_i},去训练学生网络参数
% \subsubsection{Knowledge Distillation Module}
\subsubsection{Knowledge Distillation Mechanism}
As introduced above, the teacher module learns to allocate the team reward reasonably by taking full advantage of the global information while the student module focuses on learning a reasonable individual local Q-value to realize decentralized execution.
To bridge the teacher module and the student module, we employ the knowledge distillation mechanism, $i.e.$, distilling the perfect action-value $\hat{Q}_i$ estimated by the teacher model to guide the student module to approximate the local Q-value.
Specifically, we adopt a mean-squared-error loss (MSE) to minimize the difference between the Q-values estimated by these two modules.
% In order to distill the knowledge learned by the teacher model to the student model, we employ a mean-squared-error loss (MSE) to guide the student model to approximate the perfect action-value $\hat{Q}_i$ estimated by the teacher model as much as possible.
The advantage of MSE is that it constrains the complete set of action-value in the student model~\cite{rusu2016policy}.
Formally, the MSE loss is calculated as follows:
\begin{equation}
    L_{\text{MSE}} = \Sigma_{i=1}^{n}\Sigma_{a \in A}(\hat{Q}_i(\hat{\tau_i},a)-Q_i(\tau_i,a))^2.
\end{equation}

\subsubsection{Training and Execution}
% In the training phase, the action of each agents required to interact with the environment is generated by the teacher module, and the parameters of the teacher module and the student module are trained at the same time with the data generated by the interaction.
In the training phase, the teacher module generates the corresponding actions of each agent based on the centralized observations to interact with the environment.
Formally, the interactive actions are the results of the $\epsilon$-greedy from the $\hat{Q}_i$, which means choosing random actions with probability $\epsilon$, otherwise choosing actions with the maximal $\hat{Q}_i$.
The parameters of the teacher module and the student module are updated at the same time through iterative interactions.
The teacher module is optimized under the constraint of TD loss while the student module learns the parameters with MSE loss.
% the action of each agents required to interact with the environment is generated by the teacher module, and the parameters of the teacher module and the student module are trained at the same time with the data generated by the interaction.
% In the execution phase, only the decentralized student module is executed.
The execution phase only relies on the decentralized student module which utilizes the local action-observation records. 
To be concrete, each agent chooses a greedy action $a_i^t$ at each timestamp with respect to the individual Q-value $Q_i$ estimated by the student module.
% Each agent choosing greedy actions $a_i$ with respect to $Q_i$.
Therefore, the CTDS framework still meets centralized training and decentralized execution.
For better understanding, we provide detailed procedure of our framework below.

%CTDS的好处
% \begin{table*}[!]
% 	\centering
% 	\resizebox{\textwidth}{!}{
% 	\renewcommand{\arraystretch}{1.5}
% 	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}% 
% 		\hline
% 		\multirow{2}{*}{Scenario}   & \multicolumn{3}{|c|}{VDN\cite{sunehag2017value}} & \multicolumn{3}{|c|}{QMIX\cite{rashid2018qmix}} & \multicolumn{3}{|c|}{QPLEX\cite{wang2020qplex}}\\
% 		\cline{2-10}
% 		 &Baseline & Teacher & Student & Baseline & Teacher & Student & Baseline & Teacher & Student\\
% 		\hline
% 		5m\_vs\_6m & 6.9 $\pm$ 0.2 & 73.8 $\pm$ 0.9 & \textbf{55.0 $\pm$ 0.5} & 21.2 $\pm$ 0.4 & 66.9 $\pm$ 0.5 & \textbf{48.1 $\pm$ 1.0} & 23.8 $\pm$ 1.4 & 62.5 $\pm$ 0.9 & \textbf{56.2 $\pm$ 3.7}\\
% 		2c\_vs\_64zg & 44.4 $\pm$ 4.7 & 70.6 $\pm$ 3.6 & \textbf{57.5 $\pm$ 2.6} & 69.4 $\pm$ 2.6 & 82.5 $\pm$ 0.4 & \textbf{80.6 $\pm$ 0.7} & 81.9 $\pm$ 0.6 & 93.1 $\pm$ 0.1 & \textbf{87.5 $\pm$ 0.4}\\
% 		bane\_vs\_bane &  \textbf{76.9 $\pm$ 7.7} & 37.5 $\pm$ 3.6 & 47.5 $\pm$ 1.0 & 56.2 $\pm$ 18.6 & 67.5 $\pm$ 13.5 & \textbf{63.1 $\pm$ 12.0} & \textbf{91.9 $\pm$ 0.8} & 90.6 $\pm$ 0.6 & 71.2 $\pm$ 8.0\\	
		
% 		27m\_vs\_30m & 0.0 $\pm$ 0.0 & 6.2 $\pm$ 0.1 & \textbf{1.9 $\pm$ 0.0} & 8.8 $\pm$ 1.0 & 58.8 $\pm$ 2.4 & \textbf{42.5 $\pm$ 1.5} & 0.0 $\pm$ 0.0 & 60.9 $\pm$ 5.8 & \textbf{49.2 $\pm$ 8.9}\\
% 		MMM2 & 0.0 $\pm$ 0.0 & 15.6 $\pm$ 1.2 & \textbf{2.5 $\pm$ 0.1} & 20.6 $\pm$ 1.2 & 80.6 $\pm$ 1.7 & \textbf{28.1 $\pm$ 1.7} & 0.0 $\pm$ 0.0 & 26.6 $\pm$ 0.8 & \textbf{1.6 $\pm$ 0.1}\\
% 	    6h\_vs\_8z& 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 &0.0 $\pm$ 0.0& 0.0 $\pm$ 0.0 & 8.1 $\pm$ 2.6 & 0.0 $\pm$ 0.0\\
% 	    3s5z\_vs\_3s6z& 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 1.2 $\pm$ 0.0 & 0.0 $\pm$ 0.0&  0.0$\pm$ 0.0& 3.8 $\pm$ 0.4 & 0.0 $\pm$ 0.0\\
% 	    corridor& 0.6 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$  0.0 & \textbf{1.2 $\pm$ 0.0} & 0.0$\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 16.9 $\pm$ 10.4 & \textbf{1.2 $\pm$ 0.0}\\
% 		\hline
% 		Average & 16.1  & 25.5 & \textbf{20.6}  & 22.2 & 44.7 & \textbf{32.8} & 24.7 & 45.3 & \textbf{33.4} \\
% 		\hline
% 	\end{tabular}}
% 	% \caption{Mean and variance performance of the test win percentage in different scenarios.}
% 	\caption{The performance of the test win rate percentage (including mean and standard deviation) of different base models under different scenarios after training 2M steps.
% 	``Baseline'' represents the original base model; ``Teacher'' and ``Student'' represent the teacher and student module of CTDS, respectively.
% 	The one with the higher win rate of ``Student'' and ``Baseline'' is highlighted with bold.
% 	}
% 	\label{tab:result}
% \end{table*}

\subsection{Theoretical Analysis}\label{sec:anal}
In this subsection, we theoretically derive why the student module performs better than the execution module of CTDE with the equivalent input information. 

As mentioned above, the teacher module learns from the centralized history trajectory $\hat{\tau}_i$, which contains the decentralized information ${\tau}_i$ (accessible to the student module) and the complement information $\tau^*_i=\hat{\tau}_i^t\setminus{\tau}_i^t$ (we assume that $\tau_i$ and $\tau^*_i$ are independent).
In order to explain the relationship between input trajectories and output individual Q-values more clearly, we simplify the student module and teacher module into the following formulation:
\begin{equation}
\begin{aligned}
    (\text{Teacher network})\qquad &f_{T}:(\tau_i, \tau^*_i)\rightarrow \hat{Q}_i,\\
    (\text{Student network})\qquad &f_{S}:\tau_i\rightarrow Q_i.
\end{aligned}
\end{equation}
The student module of CTDS and the execution module of CTDE both employ decentralized information merely. 
Due to the limitation of partial trajectory, $i.e.$, the lack of $\tau^*_i$, the execution module of CTDE tends to make non-optimal actions for the current state.
The centralized trajectory releases the restriction above, however, it's usually unavailable during execution. 

CTDS takes both sides into consideration. For a certain decentralized trajectory ${\tau}_i$, the teacher module can give a centralized Q-value $f_T(\tau_i, \tau^*_i)$ with any possible implicit knowledge $\tau^*_i$. 
If the expectation of teacher module's output on implicit information $\mathbb{E}_{\tau^*_i} f_T(\tau_i, \tau^*_i)$ is achieved, it can be used to instruct student module $f_S$ to reduce environment uncertainty caused by the partial trajectory. 
Nevertheless, approximating $\mathbb{E}_{\tau^*_i} f_T(\tau_i, \tau^*_i)$ directly needs a large number of centralized trajectory samples, which is computationally expensive.

The following theorem proves that CTDS framework successfully employs $\mathbb{E}_{\tau^*_i} f_T(\tau_i, \tau^*_i)$ to train student module. 
The comprehensiveness and stability provided by the instruction from the teacher module is the principal cause of the student module's performance promotion.

\textbf{Theorem 1.} For any decentralized trajectory ${\tau}_i$, the student module of CTDS
$f_{S}(\tau_i)$ is instructed to approximate the expectation of a centralized Q-value function  on implicit information $\mathbb{E}_{\tau^*_i} f_T(\tau_i, \tau^*_i)$.

\emph{Proof:}
With a fixed teacher network, the optimization target of student network is
\begin{equation}
    \mathop{\arg\min}_{\theta_S} \ \ \sum\nolimits_{i}\mathbb{E}_{\tau_i, \tau^*_i}
    [f_S(\tau_i)-f_T(\tau_i, \tau^*_i)]^2,
\end{equation}
where $\theta_S$ is the parameters of the student module. It can be proven that:
\begin{equation}
\begin{aligned}
    & \ \ \ \ \frac{\partial}{\partial \theta_S}\mathbb{E}_{\tau^*_i}
    [f_S(\tau_i)-f_T(\tau_i, \tau^*_i)]^2\\ 
    &= \frac{\partial}{\partial \theta_S}\int [f_S(\tau_i)-f_T(\tau_i, \tau^*_i)]^2 p(\tau^*_i) d\tau^*_i \\
    &= \int 2(f_S(\tau_i)-f_T(\tau_i, \tau^*_i)) p(\tau^*_i) \frac{\partial f_S(\tau_i)}{\partial \theta_S} d\tau^*_i \\
    &= 2\frac{\partial f_S(\tau_i)}{\partial \theta_S}[f_S(\tau_i)- \int f_T(\tau_i, \tau^*_i)) p(\tau^*_i) d\tau^*_i]\\
    &= \frac{\partial}{\partial \theta_S}[f_S(\tau_i)- \int f_T(\tau_i, \tau^*_i)) p(\tau^*_i) d\tau^*_i]^2\\
    &= \frac{\partial}{\partial \theta_S}[f_S(\tau_i)- \mathbb{E}_{\tau^*_i} f_T(\tau_i, \tau^*_i)]^2\\
\end{aligned}
\end{equation}
Therefore, 
\begin{equation}
\begin{split}
  \mathop{\arg\min}_{\theta_S}  \sum\nolimits_{i}\mathbb{E}_{\tau_i, \tau^*_i}
    [f_S(\tau_i)-f_T(\tau_i, \tau^*_i)]^2 
    = \mathop{\arg\min}_{\theta_S}  \sum\nolimits_{i}\mathbb{E}_{\tau_i}
    [f_S(\tau_i)- \mathbb{E}_{\tau^*_i} f_T(\tau_i, \tau^*_i)]^2.
\end{split}
\end{equation}




\section{Experiments}
In this section, we conduct comprehensive experiments to demonstrate the effectiveness of our method. 
% We evaluate CTDS in the StarCraft II decentralized micromanagement tasks and
% use StarCraft Multi-Agent Challenge (SMAC) environment \cite{samvelyan19smac} as our testbed, which has become a commonly-used benchmark for evaluating state-of-the-art MARL approaches.
All of the following experiments are to prove that our approach is robust enough to work on a variety of tasks.
Our codes are available in https://github.com/cathyhxh/CTDS.




\subsection{Settings}\label{sec:set}
%We conduct experiments on StarCraft II decentralized micromanagement tasks to evaluate the effectiveness of our method.

In this paper, we test our method on two environments: Combat (a grid world environment introduced by~\cite{magym}) and StarCraft II micromanagement (SMAC)~\cite{samvelyan19smac}.


\begin{figure}[t]
	\centering
	\subfigure[Combat]{
		\includegraphics[width=0.17\columnwidth]{combat.png}
	}
	\subfigure[SMAC]{
		\includegraphics[width=0.17\columnwidth]{smac.jpg}
	}
	\subfigure[with sight range limit]{
		\includegraphics[width=0.25\columnwidth]{with_sight_range.pdf}
		\label{fig2-1}
	}
	\subfigure[without sight range limit]{
		\includegraphics[width=0.25\columnwidth]{without_sight_range.pdf}
		\label{fig2-2}
	}
	\label{fig:sight}
	\caption{(a)\&(b) Visualisation of the two experimental environments. (c)\&(d) An illustration about the agents with partial and global observation in SMAC.}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 		\subfigure[with sight range limit]{
% 		\includegraphics[width=0.25\columnwidth]{with_sight_range.pdf}
% 		\label{fig2-1}
% 	}
% 	\subfigure[without sight range limit]{
% 		\includegraphics[width=0.25\columnwidth]{without_sight_range.pdf}
% 		\label{fig2-2}
% 	}
% 	\caption{An illustration about the agents with partial and global observation in SMAC.}
% 	\label{fig:ob}
% \end{figure}

\begin{figure*}[t]
	\centering
	\subfigure[VDN-5m\_vs\_6m]{
		\includegraphics[width=0.22\textwidth]{vdn_5m_vs_6m.pdf}
		\label{VDN-5m\_vs\_6m}
	}
	\hfill
	\subfigure[QMIX-5m\_vs\_6m]{
		\includegraphics[width=0.22\textwidth]{qmix_5m_vs_6m.pdf}
		\label{QMIX-5m\_vs\_6m}
	}
	\hfill
	\subfigure[QPLEX-5m\_vs\_6m]{
		\includegraphics[width=0.22\textwidth]{qplex_5m_vs_6m.pdf}
		\label{QPLEX-5m\_vs\_6m}
	}
	\hfill
	\subfigure[VDN-bane\_vs\_bane]{
		\includegraphics[width=0.22\textwidth]{vdn_bane_vs_bane.pdf}
		\label{VDN-bane\_vs\_bane}
	}
	\newline
	\subfigure[QMIX-bane\_vs\_bane]{
		\includegraphics[width=0.22\textwidth]{qmix_bane_vs_bane.pdf}
		\label{QMIX-bane\_vs\_bane}
	}
	\hfill
	\subfigure[QPLEX-bane\_vs\_bane]{
		\includegraphics[width=0.22\textwidth]{qplex_bane_vs_bane.pdf}
		\label{QPLEX-bane\_vs\_bane}
	}
	\hfill
	\subfigure[VDN-27m\_vs\_30m]{
		\includegraphics[width=0.22\textwidth]{vdn_27m_vs_30m.pdf}
		\label{VDN-27m\_vs\_30m}
	}
	\hfill
	\subfigure[QMIX-27m\_vs\_30m]{
		\includegraphics[width=0.22\textwidth]{qmix_27m_vs_30m.pdf}
		\label{QMIX-27m\_vs\_30m}
	}
	\newline
	\subfigure[QPLEX-27m\_vs\_30m]{
		\includegraphics[width=0.22\textwidth]{qplex_27m_vs_30m.pdf}
		\label{QPLEX-27m\_vs\_30m}
	}
	\hfill
	\subfigure[VDN-MMM2]{
		\includegraphics[width=0.22\textwidth]{vdn_MMM2.pdf}
		\label{VDN-MMM2}
	}
	\hfill
	\subfigure[QMIX-MMM2]{
		\includegraphics[width=0.22\textwidth]{qmix_MMM2.pdf}
		\label{QMIX-MMM2}
	}
	\hfill
	\subfigure[QPLEX-MMM2]{
		\includegraphics[width=0.22\textwidth]{qplex_MMM2.pdf}
		\label{QPLEX-MMM2}
	}
	\newline
	\subfigure[VDN-2c\_vs\_64zg]{
		\includegraphics[width=0.22\textwidth]{vdn_2c_vs_64zg.pdf}
		\label{VDN-2c\_vs\_64zg}
	}
	\hfill
	\subfigure[QMIX-2c\_vs\_64zg]{
		\includegraphics[width=0.22\textwidth]{qmix_2c_vs_64zg.pdf}
		\label{QMIX-2c\_vs\_64zg}
	}
	\hfill
	\subfigure[QPLEX-2c\_vs\_64zg]{
		\includegraphics[width=0.22\textwidth]{qplex_2c_vs_64zg.pdf}
		\label{QPLEX-2c\_vs\_64zg}
	}
	\hfill
	\subfigure{
		\includegraphics[width=0.2\textwidth]{tuli.pdf}
		\label{legand}
	}
	\caption{
	Test win rates of the base models ($i.e.$, VDN,  QMIX  and  QPLEX)  and the corresponding ones with CTDS algorithm on five different maps of StarCraft II.
	``Baseline'' represents the performance of the original base model; ``Teacher'' and ``Student'' represent the performance of teacher and student module of CTDS, respectively.
	``Baseline'' and ``Student'' achieve decentralized execution.	
	The solid/dashed line shows the median win rate and the shadow area represents the max-min win rate in 5 different random seeds.}
	\label{Experiment}
\end{figure*}

 In the experiment implementation, the different between partial observation and perfect observation depends on the sight range setting. 
 Partial observation restricts the agents from receiving information about allied or enemy units that are out of range, $i.e.$, the features of enemies and allies are all unknown when the corresponding unit beyond the sight range.
For example, the sight range of each agent is set to 2, which means each agent is allowed to only access its own features and other units' features within the distance of 2.
For the teacher module, perfect observation $\hat{o}_i$ is not limited by the sight range, that is to say, each agent can access the full observation of all the agents.
Figure3 shows the examples of the agent with partial and global observations in the SMAC, respectively.
In SMAC, we set partial sight range as 2 and perfect sight range as infinity.
In Combat, partial sight range is 2 and perfect sight range is 4.

\begin{table*}[t]
	\centering
	\resizebox{\textwidth}{!}{
	\renewcommand{\arraystretch}{1.5}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}% 
		\hline
		\multirow{2}{*}{Scenario}  & \multicolumn{3}{|c|}{VDN\cite{sunehag2017value}} & \multicolumn{3}{|c|}{QMIX\cite{rashid2018qmix}} & \multicolumn{3}{|c|}{QPLEX\cite{wang2020qplex}}\\
		\cline{2-10}
		 &Baseline & Teacher & Student & Baseline & Teacher & Student & Baseline & Teacher & Student\\
		\hline
		5m\_vs\_6m & 6.9 $\pm$ 0.2 & 73.8 $\pm$ 0.9 & \textbf{55.0 $\pm$ 0.5} & 21.2 $\pm$ 0.4 & 66.9 $\pm$ 0.5 & \textbf{48.1 $\pm$ 1.0} & 23.8 $\pm$ 1.4 & 62.5 $\pm$ 0.9 & \textbf{56.2 $\pm$ 3.7}\\
		9m\_vs\_11m & 0.6 $\pm$ 0.0 & 9.4 $\pm$ 0.6 & \textbf{12.5 $\pm$ 1.1} & 6.9 $\pm$ 0.1 & 9.4 $\pm$ 0.2 & \textbf{11.2 $\pm$ 0.1} & \textbf{3.1 $\pm$ 0.1} & 0.6 $\pm$ 0.0 & 0.6 $\pm$ 0.0 \\
		27m\_vs\_30m & 0.0 $\pm$ 0.0 & 6.2 $\pm$ 0.1 & \textbf{1.9 $\pm$ 0.0} & 8.8 $\pm$ 1.0 & 58.8 $\pm$ 2.4 & \textbf{42.5 $\pm$ 1.5} & 0.0 $\pm$ 0.0 & 60.9 $\pm$ 5.8 & \textbf{49.2 $\pm$ 8.9}\\
		MMM2 & 0.0 $\pm$ 0.0 & 15.6 $\pm$ 1.2 & \textbf{2.5 $\pm$ 0.1} & 20.6 $\pm$ 1.2 & 80.6 $\pm$ 1.7 & \textbf{28.1 $\pm$ 1.7} & 0.0 $\pm$ 0.0 & 26.6 $\pm$ 0.8 & \textbf{1.6 $\pm$ 0.1}\\
		2c\_vs\_64zg & 44.4 $\pm$ 4.7 & 70.6 $\pm$ 3.6 & \textbf{57.5 $\pm$ 2.6} & 69.4 $\pm$ 2.6 & 82.5 $\pm$ 0.4 & \textbf{80.6$\pm$ 0.7} & 81.9 $\pm$ 0.6 & 93.1 $\pm$ 0.1 & \textbf{87.5 $\pm$ 0.4}\\
		\hline
		Average & 10.4  & 35.1 & \textbf{25.9}  & 25.4 & 59.6 & \textbf{42.1} & 21.8 & 48.7 & \textbf{39.0} \\
		\hline
	\end{tabular}}
	% \caption{Mean and variance performance of the test win percentage in different scenarios.}
	\caption{The performance of the test win rate percentage (including mean and standard deviation) of different base models under different scenarios of StarCraft II.
	``Baseline'' represents the original base model; ``Teacher'' and ``Student'' represent the teacher and student module of CTDS, respectively.
	The one with higher win rate of ``Student'' and ``Baseline'' is highlighted with bold.
	}
	\label{tab:result}
\end{table*}

% \textbf{Combat:}
% We simulate a simple battle in a $7 \times 7$ grid with two opposing teams (red team and blue team). 
% In each time step, agents in each team has three possible actions: move, attack, or do nothing.
% If all the agents in a team die, the other team wins.
% We need to control a whole team in training, and the opponent team is controlled by a hard-coded strategy. 
% It is worth noting that the opponent team is view-shared, $i.e.$ if a agent is visible, it will appear in the view of other opponent agents. 
% It gives the opponent team a considerable advantage over our team.
% % In this environment, the sight range of each agent is set to 2, which is set to 4 in the teacher module.

% \textbf{SMAC:}
% SMAC has become a commonly-used benchmark for evaluating state-of-the-art MARL approaches.
% The experiments are carried out in hard  and  super hard maps proposed in \cite{samvelyan19smac}. 
% In these tasks, the observation of each agent consists of three parts, which are its own features, enemy features and ally features. 
% Partial observation restricts the agents from receiving information about allied or enemy units that are out of range, $i.e.$, the features of enemies and allies are all 0 when the corresponding unit beyond the sight range.
% In this paper, the sight range of each agent is set to 2, which means each agent is allowed to only access its own features and other units' features within the distance of 2.

% For the teacher module, perfect observation $\hat{o}_i$ is not limited by the sight range, that is to say, each agent can access the full observation of all the agents.
% Figure~\ref{fig:ob} shows the examples of the agent with partial and global observations, respectively.

The algorithms we use are based on the Pymarl algorithm library \cite{samvelyan19smac}.
To reduce randomness, all the reported results are averaged over 5 runs with different seeds.
Training and evaluation schedules such as the testing episode number and training hyper-parameters are kept the same as default hyper-parameters in Pymarl.
Following the base models~\cite{sunehag2017value,rashid2018qmix,wang2020qplex}, we share the parameters of the agent networks across all agents in the teacher/student module to speed up the learning.
Note that the parameters of the teacher module and student module are not shared.
All the parameters in the neural networks are adjusted by a RMSprop optimizer with a learning rate of 0.0005, the same as that used by the baselines.
% The parameters in teacher module and student module are adjusted by a RMSprop optimizer, and its learning rate, alpha, epsilon are 0.0005, 0.99, 0.00001, respectively.
For all the compared methods, each task is trained for 2 Million steps separately in SMAC and 500k steps in Combat.

% \subsection{Validation}
\subsection{Performance Evaluation and Discussion}\label{sec:eval}
Our CTDS framework can be applied upon various existing models that follow the CTDE paradigm.
To show the effectiveness of our CTDS framework, we conduct the experiments upon three representative models with different mixing network settings: VDN \cite{sunehag2017value}, QMIX \cite{rashid2018qmix} and QPLEX \cite{wang2020qplex}.
% We compare the performance of CTDS with previous CTDE algorithm in Under two different mixing network settings: VDN \cite{sunehag2017value}, QMIX \cite{rashid2018qmix} and QPLEX \cite{wang2020qplex}.

% Table~\ref{tab:result} shows the final mean and variance performance of the test win percentage under different scenarios.



\begin{figure*}[h]
	\centering
	\subfigure[QMIX]{
		\includegraphics[width=0.4\textwidth]{qmix_Combatwrapped4-chosen.pdf}
	}
	\subfigure[QPLEX]{
		\includegraphics[width=0.4\textwidth]{qplex_Combatwrapped4-chosen.pdf}
	}
	\caption{Test win rates of the base models (QMIX and QPLEX) and the corresponding ones with CTDS algorithm in Combat. “Baseline” represents the performance of the original base model; “Teacher” and “Student”represent the performance of teacher and student module of CTDS, respectively. “Baseline” and “Student” achieve decentralized execution. The solid/dashed line shows the median win rate and the shadow area represents the max-min win rate in 5 different random seeds. }
	\label{fig:combat_results}
\end{figure*}


First we conduct the experiment in grid world environment Combat.
The Figure \ref{fig:combat_results} reveals the test win rate curves of CTDS and baselines under the settings of the mixing neural network of QMIX and QPLEX after 500k steps of training.
As demonstrated in Figure \ref{fig:combat_results}, the CTDE paradigm  improves convergence speed at the beginning of trainning and reaches the converging win rate with much lower variance.

The following are the experiment results in StarCraft II.
Table~\ref{tab:result} shows the final performance in terms of the test win rate percentage criteria of different base models under different scenarios.
Here ``Baseline'' means the performance of the original base model which achieves decentralized execution; ``Teacher'' means the performance of the teacher module which relies on the perfect observation thus violates decentralized execution; ``Student'' means the performance of the student module, which distills the knowledge from the teacher and allows decentralized execution.

It can be seen that the teacher always achieves a higher win percentage than the student, which is consistent with our assumption that the full observation brings benefits.
% 这句话得改 + 补充
Under the settings of the mixing neural network of VDN, QMIX and QPLEX, after 2 million steps of training, the performance gap between CTDS and the baseline exceeds the average win rate of 15.5\%, 16.7\% and 17.2\%, respectively.
% Noting that the test win rates of the student and the teacher module are both lower than baseline with mixing network setting QPLEX under scenarios 9m\_vs\_11m. 
% The final experimental results are shown in Figure \ref{Experiment}.
Figure~\ref{Experiment} demonstrates the learning curve of the base model, the teacher module and the student module on different scenarios.
% 待讨论
% It is observed that the teacher module consistently learns the fastest and the following is the student module.
%Compared to the base model, the extra time cost of jointly training of the teacher module and the student module is little.
%In addition, the stability of the training process is similar to the base model, which indicates the robustness of our framework.
% The above results indicate that CTDS framework can boost the performance of the original algorithms to a considerable margin in most scenarios, and can accelerate training as well.
The above results indicate that CTDS framework can boost the performance of the original algorithms to a considerable margin in most scenarios.

% \subsection{Efficiency Analysis}\label{sec:effi}
% Compared to the base model, our CTDS framework requires to jointly train the teacher module and the student module, which will increase the time cost.
% In this section, we further investigate how much extra time that CTDS introduces.
% All the efficiency experiments are conducted on a Ubuntu 18.04 sever with 4 Intel(R) Xeon(R) Gold 6252 CPU @ 2.10GHz and GeForce RTX 2080Ti GPU.

% % 训练配置 to do
% Table~\ref{tab:time} illustrates the time cost of the three base models and the corresponding CTDS methods on different maps.
% We can see that applying CTDS over the base model brings about around 30\% extra time cost on average.
% The reason is that compared to the teacher module, which has a similar network as the base model, the student module has a much simpler network structure with fewer trainable parameters.


% \begin{table*}[htbp]
% 	\centering
% 	\resizebox{\textwidth}{!}{
% 	\renewcommand{\arraystretch}{1.25}
% 	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}% 
% 		\hline
% 		\multirow{2}{Scenario} & \multicolumn{3}{|c|}{VDN\cite{sunehag2017value}} & \multicolumn{3}{|c|}{QMIX\cite{rashid2018qmix}} & \multicolumn{3}{|c|}{QPLEX\cite{wang2020qplex}}\\
% 		\cline{2-10}
% 		 &Baseline & CTDS & Rate & Baseline & CTDS & Rate & Baseline & CTDS & Rate\\
% 		\hline
% 		5m\_vs\_6m  & 112.0 & 147.5 & 31.7\% & 119.8 & 155.8   & 30.0\% & 134.8 & 159.8  & 18.5\%\\
% 		9m\_vs\_11m & 131.8  & 180.7 & 37.1\%  & 153.9 & 211.7 & 37.6\% & 179.7& 204.8  & 14.0\% \\
% 		27m\_vs\_30m & 272.7& 389.9  & 43.0\% & 296.2 & 384.8 & 29.9\% & 286.6 & 438.3 & 52.9\%\\
% 		MMM2 & 162.5& 212.3  & 30.6\% & 160.7& 178.7  & 11.2\% & 164.0 & 218.6 & 33.3\%\\
% 		2c\_vs\_64zg & 201.7 & 243.3 & 20.6\% & 208.7 & 249.5 & 19.5\% & 209.9& 280.4  & 33.6\%\\
% 		\hline
% 		Average & \diagbox[dir=SW]{}{}  & \diagbox[dir=SW]{}{}& 32.6\%  &\diagbox[dir=SW]{}{}  & \diagbox[dir=SW]{}{}& 25.7\% & \diagbox[dir=SW]{}{}  & \diagbox[dir=SW]{}{}& 30.2\%  \\
% 		\hline
% 	\end{tabular}}
% 	% \caption{Mean and variance performance of the test win percentage in different scenarios.}
% 	\caption{The time(seconds) required to train 10k steps for different base models and the corresponding CTDS methods under different scenarios.
% 	``Baseline'' represents the original base model and ``CTDS'' represents the corresponding method in our framework.  
% 	``Rate'' means the extra time cost percentage of CTDS compared with baselines.
% 	%``B" represents the performance of the baseline, ``T" represents the teacher model and ``S" represents the student model.
% 	}
% 	\label{tab:time}
% \end{table*}

\subsection{Sight Range Analysis}


Under the setting of partial observability, agents can only receive the information within the restricted sight range.
All the results reported in Section~\ref{sec:eval} are under the scenario that the sight range is 2.
In this section, we further analyze the generalization of our method with regard to different sight ranges.
% \vspace{-0.3cm}
\begin{wrapfigure}{r}{0.55\textwidth}
	\centering
    \setlength{\abovecaptionskip}{-0.2cm}
	\includegraphics[width=0.55\textwidth]{ablation_mean.pdf}
	\caption{The performance of the test win rate percentage (including mean and standard deviation) of the different sight range. 
	The experiment takes QMIX as the base model on the 2c\_vs\_64zg task after 1 million steps of training. ``Baseline'' represents the performance of the original base model which achieves decentralized execution; ``Teacher'' and ``Student'' represent the performance of teacher and student module of CTDS, respectively.}
	\label{ablation}
\end{wrapfigure}

% \begin{wrapfigure}{r}{0.5\textwidth}
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{Figure/ablation_mean.pdf}
% 	\caption{The performance of the test win rate percentage (including mean and standard deviation) of the different sight range. 
% 	The experiment takes QMIX as the base model on the 2c\_vs\_64zg task after 1 million steps of training. ``Baseline'' represents the performance of the original base model which achieves decentralized execution; ``Teacher'' and ``Student'' represent the performance of teacher and student module of CTDS, relatively.}
% 	\label{ablation}
% \end{wrapfigure}
We adjust the sight range from 1 to 8 in the environment, and investigate the performance of the base model, the teacher module and the student module under each setting, respectively.
% While testing, we adjust the different sight range in the environment, respectively, and report the results under each setting for better analysis.
Due to the page limit, we only represent the results of methods taking QMIX as the base model on the 2c\_vs\_64zg task of StarCraft II after 1 million steps of training.
As illustrated in Figure~\ref{ablation}, we can see that the performance of the original QMIX significantly increases with the increasing sight range, which indicates that more information about the other agents brings about a higher win percentage.
Besides, the margin gain of the win percentage with one more sight range shows a decreasing trend,
% and the win percentage gains the largest margin from the setting that agents can only see their own features to that agents can also see the enemy features, 
which is consistent with our common sense.
Different from the base model which relies heavily on the sight range, the performance of our CTDS framework is relatively stable under different sight range that increases at a lower margin as the sight range enlarges.
In other words, the performance gap between CTDS and the baseline increases with the decrease of sight range from 8 to 1.
Our CTDS framework thereby has remarkable advantages in the case of the very limited observations.
Overall, the generalization of our framework with the varying of sight range indicates the efficacy of the knowledge distillation mechanism.

% For example, in Figure \ref{ablation}, we can see the trend of performance with the change of the sight range from 1 to 8 in the 2c\_vs\_64zg task and QMIX mixing network setting.
% In Figure \ref{ablation}, the performance gap between CTDS and the baseline increases with the decrease of sight range from 8 to 1.
% Those can be concluded that CTDS algorithm has better performance in the case of more limited observations.

